Rich-Item Recommendations for Rich-Users: Exploiting Dynamic and Static Side Information

In this paper, we study the problem of recommendation system where the users and items to be recommended are rich data structures with multiple entity types and with multiple sources of side-information in the form of graphs. We provide a general formulation for the problem that captures the complexities of modern real-world recommendations and generalizes many existing formulations. In our formulation, each user/document that requires a recommendation and each item or tag that is to be recommended, both are modeled by a set of static entities and a dynamic component. The relationships between entities are captured by several weighted bipartite graphs. To effectively exploit these complex interactions and learn the recommendation model, we propose MEDRES- a multiple graph-CNN based novel deep-learning architecture. MEDRES uses AL-GCN, a novel graph convolution network block, that harnesses strong representative features from the underlying graphs. Moreover, in order to capture highly heterogeneous engagement of different users with the system and constraints on the number of items to be recommended, we propose a novel ranking metric pAp@k along with a method to optimize the metric directly. We demonstrate effectiveness of our method on two benchmarks: a) citation data, b) Flickr data. In addition, we present two real-world case studies of our formulation and the MEDRES architecture. We show how our technique can be used to naturally model the message recommendation problem and the teams recommendation problem in the Microsoft Teams (MSTeams) product and demonstrate that it is 5-6% points more accurate than the production-grade models.

==> abstract.tex <==
In this paper, we study the problem of recommendation system with multiple entity types and with side-information in the form of multiple graphs. We provide a general formulation for the problem that captures the complexities of modern real-world recommendations and generalizes many existing formulations. In our formulation,  each user/document that requires a recommendation is modeled by a set of static entities and a dynamic component. Similarly, each item/tag to be recommended is also modeled by a set of static entities and a dynamic component. The relationships between entities are captured by several weighted bipartite graphs. To effectively exploit these complex interactions and learn the recommendation model, we propose \medres -- a multiple graph-CNN based novel deep-learning architecture. 
% , which effectively exploits complex interactions and learns the recommendation model. 
Further, our architecture focuses on a new metric that is critical in certain classification+ranking scenarios. We demonstrate effectiveness of our method on two benchmarks: a) citation data, b) Flickr data. In addition, we present a case study of how our formulation and method can be used to model the message recommendation problem in the Microsoft Teams (MSTeams) product. In particular, we show that our technique can improve the existing production-grade model by 5-6\% points.

==> exps.tex <==
%\section{Experiments Setup}
\label{sec:exps}

%\input{exps}
We now demonstrate the wide-applicability and effectiveness of our method on three problems from disparate domains. These are: (a) message recommendation system for Microsoft Teams (aka message-reco), (b) citation recommendation for research papers (aka citation-reco), and (c) group recommendation for photos (aka group-reco). 

\subsection{Datatsets}
\textbf{Message-Reco:} The task is to predict the relevance of a given message for a given user. This problem commonly arise in notification or activity feed systems such as in MSTeams. Each message is associated with three static and one dynamic entity. Static entities are: (a) user consuming the message, (b) author of the message, and (c) channel where the message is posted. Dynamic entity is the content of the message. We consider six months of interaction data to construct graphs between static entities. This gives us 23 directed graphs between users and authors, e.g. messages sent from user to author, numbers of actions such as likes by a user on an author's messages, etc. Similarly, we have 12 directed graphs between users and channels, e.g. how many times a user posted on a channel, how many times a user liked a message posted on a channel, etc. We then collect data from the next 4 weeks of logs from MSTeams and label a (user, message)-tuple to be positive if a user engages with the message in some manner and mark it to be negative otherwise. We divide our collected data, i.e., labeled user-message tuples into train, validation, and test datasets where two weeks of data is used for training, onw week for validation, and one week's data for test. Further statistics about the dataset are mentioned in Table \ref{teams_data_stats}.


\begin{table*}
\centering
	\caption{Teams Message Recommendation Dataset Statistics}
	\label{teams_data_stats}
\begin{tabular}{|l|l|l|l|}
\hline
Statistic        & Training Data & Val Data & Test Data \\ \hline
Number of points & 3416632       & 379626   & 1499083   \\ \hline
\% of positives  & 4.40          & 4.87     & 4.80      \\ \hline
Users            & 901           & 898      & 898       \\ \hline
Authors          & 677           & 509      & 593       \\ \hline
Channels         & 476           & 367      & 391       \\ \hline
\end{tabular}
\end{table*}






\textbf{Citation-Reco:} For the citation-reco. problem, we extract data from the Citation-network V1 -- a publicly available dataset \cite{Tang:08KDD}. 
The goal of the problem is to recommend relevant citations for a paper being written. The static entities in this problem are - users who are writing a new paper, authors of the already published papers, and conferences where the candidate recommendations have been published; the title and abstract of the paper being written and the one that is being considered for recommendation are dynamic entities. For creating entity graphs and training data, we use citation data from 1998-2002. The validation and test datasets are created using citation data from 2003 and 2004-2005, respectively. We consider 3 graphs between users and authors for co-authorship, author-cited-user and user-cited-author. For user and conferences, we consider 2 graphs - user-published-in-conference and user-cited-conference. For each paper, we embed the paper titles using $50$-dimensional GloVe~\cite{pennington2014glove} embedding vectors. For a given paper, every author and the cited paper pairs make our positive data points. If a user has cited any paper of an author in the given time window but has not cited her some other papers, then the later papers are considered as negative data points. We further sample this data such that a user and each author should have at least 20 data points in the training set. Table \ref{citation_data_stats} provides key statistics of the training and the test dataset. 


\begin{table}
\centering
\caption{Citation Recommendation Dataset Statistics}
\label{citation_data_stats}
\begin{tabular}{|l|l|l|l|}
\hline
Statistic               & Train Data & Val Data & Test Data \\ \hline
Number of points        & 238740        & 84302    & 85670     \\ \hline
\% of positives & 9.99          & 9.40     & 9.48      \\ \hline
Users         & 1602          & 962      & 1003      \\ \hline
Authors       & 1147          & 949      & 1019      \\ \hline
Conferences   & 951           & 881      & 913       \\ \hline
\end{tabular}
\end{table}
 



 
\textbf{Group-Reco:} For the group-reco. problem, we consider the openly available Flickr dataset ~\cite{wang2017flickr}. The goal of the problem is to recommend groups to a user who plans to post new photos. Each group is defined by a set of `tags' and `categories', which in layman terms are topics of the groups. For this problem, we consider 4 static entities - users, tags, categories, and groups and 3 graphs between these entities i.e. users-posted-with-tags, users-posted-in-categories, and users-posted-in-groups. We vectorize each image (dynamic component) using VGG19 ~\cite{simonyan2014very} to 4096 dimensional vectors and further apply PCA to reduce the image feature dimensions to 100. Each time a user posts in a group is considered as a positive datapoint. Negatives are generated by random sampling. Further details about the Flickr dataset are given in Table \ref{flickr_data_stats}.

\begin{table}
\centering
	\caption{Flickr Recommendation Dataset Statistics}
	\label{flickr_data_stats}
	\begin{tabular}{|l|l|l|l|}
    \hline
    Statistic        & Training Data & Val Data & Test Data \\ \hline
    Number of points & 261115        & 20139    & 59763     \\ \hline
    \% of positives  & 12.87         & 12.24    & 12.72     \\ \hline
    Users            & 839           & 205      & 439       \\ \hline
    Groups           & 464           & 422      & 453       \\ \hline
    Photos           & 3837          & 289      & 864       \\ \hline
    Entities         & 311           & 284      & 304       \\ \hline
    Categories       & 1471          & 1294     & 1413      \\ \hline
	\end{tabular}
\end{table}


\subsection{Setup}
%\vskip -.1cm
We compare our proposed MEDRES approach with two standard content-filtering baselines - LightGBM~\cite{ke2017lightgbm} and Multilayer Neural Networks (NN); later in Section~\ref{sec:exps_cf} we will compare MEDRES with a strong collaborative-filtering baseline. For both the baselines, we create  features by using the value of 1-hop edges from the graphs along with the features of the dynamic entities. The LightGBM baseline is similar to the production model. For LightGBM, we sweep on the following hyper-parameters: learning rate $\{10^{-3}, 10^{-2}\}$, number of trees $\{50, \dots, 300\}$, and number of leaves $\{10, 15, \dots, 30\}$. For the NN baseline, we sweep on the following hyper-parameters: weight regularization $\{10^{-5}, 10^{-6}$, $10^{-7}\}$, nodes in each layer $\{2^7, \dots, 2^{10}\}$, batch size $\{3, 5, 10\}\times 10^{3}$, and learning rate $\{10^{-3}, 10^{-4}\}$. For MEDRES, the cross-validation is done on embedding size $\{2^5, 2^6, 2^7\}$, 
% embedding regularization $(10^{-3}, 10^{-4})$, 
regularization parameter $\{10^{-4}, 10^{-5}\}$, nodes in fully connected layers $\{2^7, \dots, 2^{10}\}$, batch size $\{1, 3, 5\}\times 10^3$, and learning rate $\{10^{-3}, 10^{-4}\}$. We report only Micro-$\aucrelk$ (\ref{eq:microdef}) in the experiments as stated earlier in the paper, and refer it as $\aucrelk$ throughout this section. 


%\vspace{-0.5mm}

\subsection{Results}
% \vskip -0.1cm
% \setcounter{table}{2}

Figures \ref{fig:results_MEDRES}(a) reports ~\aucrelk \eqref{eq:microdef} for various methods for message-reco problem. Recall that Light-GBM model and NN model use a standard content-filtering approach where joint features for (user, message) pair are computed by concatenating standard one-hop edges from the graphs mentioned above. %For example, one such feature would be, in past, the number of times a user $\user$ liked messages from the author of message $\myitem$. 
In fact, Light-GBM is very close to the deployed production model. It can be seen that our algorithms perform significantly better than the baseline methods. For example, our method is $\approx 2.1\%$ better than the baselines in terms of \aucrelk with $k=30$. Relatively, we observe an increase of 4.41\% in \aucrelk. Note that  MEDRES also uses MLP as the final classifier, so significant gains over baseline NN (i.e. MLP) models can be directly attributed to MEDRES exploiting the graph based side-information  carefully. Figure~\ref{fig:results_MEDRES}(b) shows \aucrelk obtained by various methods with varying $k$ for the citation-reco problem.  For recommending $k=10$ articles, \medrest is $(\geq) 4.37$\% more accurate than both the baselines and similar trend holds for varying values of $k$. We observe a similar trend for the group-reco problem (see Figure~\ref{fig:results_MEDRES}(c)) where \medrest is significantly more accurate than the baseline methods. For example, for $k=5$, \medrest is 3.90\% more accurate than LGBM. 

\begin{figure*}
\begin{subfigure}{.33\textwidth}
\captionsetup{belowskip=--5pt}
  \centering
%   \hspace*{-5pt}
  \includegraphics[width=\linewidth]{figures/TeamMicro_IJCAI_2020.eps}
  \caption{}
  \label{fig:sfig1}
%   \vspace*{-5pt}
%  \vskip -0.2cm
\end{subfigure}%
\hspace*{-10pt}
\begin{subfigure}{.33\textwidth}
\captionsetup{belowskip=--5pt}
  \centering
%   \hspace*{-25pt}
  \includegraphics[width=\linewidth]{figures/Results_Citation_IJCAI_2020.eps}
  \caption{}
  \label{fig:sfig2}
%   \vspace*{-5pt}
%  \vskip -0.2cm
\end{subfigure}
\hspace*{-10pt}
\begin{subfigure}{.33\textwidth}
\captionsetup{belowskip=--5pt}
  \centering
%   \hspace*{-45pt}
  \includegraphics[width=\linewidth]{figures/Flickr_Results_IJCAI_2020.eps}
  \caption{}
  \label{fig:sfig3}
%   \vspace*{-5pt}
%  \vskip -0.2cm
\end{subfigure}
\caption{(a) Message-reco: \medreso is 2\% more accurate than baseline; optimization algorithm (Algorithm~\ref{algo}) further boosts the accuracy by $\sim 1\%$. (b) citation-reco: \medreso and \medrest are both $4-5$\% more accurate than baselines. (c)  group-reco: for $k<=6$, \medrest is about 3.5\% more accurate than baselines.}
%\vskip -0.4cm
\label{fig:results_MEDRES}
\end{figure*}

\subsection{Comparison with lesser number of graphs}
Next, we study the performance of various methods when provided with different amount of graph signals. That is, we compare the results of the LGBM (a method similar to the production model) and the MEDRES method with varying number of graphs for the message-reco dataset. Table~\ref{num_graphs_exp} shows a comparison when we use 2 graphs (1 for user-author interaction and 1 for user-channel interaction) and when we use 10 graphs (5 for user-author interactions and 5 for user-channel interactions). As we can see, MEDRES performs better by at least $2.5\%$ points when there are only 2 graphs. LGBM baseline is more severely impacted when the number of graphs are reduced to 1 each for lower k values. At $k=10$, LGBM drops from 0.468 (all 35 graphs) to 0.4471 which is approx. a $2\%$ points dip; whereas, MEDRES is more stable with a drop from 0.4731 to 0.4680 i.e. $0.5\%$ points. Thus, relatively LGBM baseline drop four times more severely than MEDRES. Moreover, the difference in LGBM baseline at $k=50$ for 10 graphs and all 35 graphs is less than $0.5\%$ points; whereas for MEDRES is more than $1\%$ points. This indicates that the production model is getting saturated earlier, but MEDRES is still able to learn more signal when more graphs are available.
\begin{table*}
	\centering
\caption{Message-reco: MEDRES is able to achieve similar accuracy as the \emph{production model} with a small number of graph signals.}
	% 	\hspace*{-30pt}
	% \vspace{4pt}
	{\small
		\begin{tabular}{|c|c|c||c|c|}
			\hline
			& \multicolumn{2}{c||}{\textbf{\#Graphs = 2 (1 each)}} &   \multicolumn{2}{c|}{\textbf{\#Graphs = 10 (5 each)}} \\ \hline
			\textbf{k}  & \textbf{LGBM}                & \textbf{MEDRES}              &   \textbf{LGBM}                & \textbf{MEDRES}               \\ \hline
			10 & 0.44710             & 0.4680              &   0.4621               & 0.4635              \\ 
			20 & 0.4484               & 0.4745              & 0.4674               & 0.4749               \\ 
			30 & 0.4517               & 0.4776                & 0.4706               & 0.4821              \\ 
			40 & 0.4511              & 0.4780                & 0.4710               & 0.4847              \\ 
			50 & 0.4524               & 0.4786                & 0.4726               & 0.4857               \\ \hline 
	\end{tabular}}
	% \vspace*{5pt}
	\label{num_graphs_exp}
\end{table*}


\subsection{Direct Embedding vs MEDRES}\label{sec:exps_cf}
% \vspace{-1.5mm}
Finally, we study the importance of the graph side-information in our architecture. As the entities are static, we can learn the embeddings  $\phi(\user)$ from scratch rather than learning it from the graph. That is, similar to collaborative filtering (CF), $\phi(\user)$ can be set to be an arbitrary vector that needs to be learned by minimizing training loss instead of constraining the vector to be generated by GCN, i.e., the system ignores the graph information completely. We refer to this method as direct embedding or non-linear CF. Intuitively, if the amount of training data is large than direct embedding should be able to learn $\phi(\user)$ accurately. However, for low-training data regime, graph information would be critical to generalize to users/items with a small amount of training data. Our experiments indeed confirm this intuition. In Table~\ref{tab:dir_emb}, we report the accuracy of both the direct embedding method as well as MEDRES on message-reco problem when trained with a varying fraction of data. Note that even when trained with all the data, Direct Embedding is  $\approx 9\%$ less accurate than MEDRES. However, the gap increases to $14\%$ when both the methods are trained with $50\%$ of the available data. This indicates that the graph information for various entities are acting as regularization and MEDRES generalizes significantly better than the  collaborative filtering architectures. 

\begin{table*}[t]
	\centering
\caption{pAp@30 for Direct Embeddings and MEDRES with different subsamples of training dataset for the message reco. dataset.}
\vskip -0.2cm
\begin{tabular}{|c|c|c|c|}
\hline
            & 50\% Data & 70\% Data & 100\% Data \\ \hline
Direct Emb. & 0.3361    & 0.3808    & 0.3966     \\ 
MEDRES      & 0.4729    & 0.4813    & 0.4892     \\ \hline
\end{tabular}
\label{tab:dir_emb}
\end{table*}

==> macros.tex <==
\newcommand{\user}{\mathcal{U}}
\newcommand{\team}{\mathcal{T}}
\newcommand{\myitem}{\mathcal{I}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\metric}{\mathcal{M}}
\newcommand{\graph}{\mathcal{G}}
\newcommand{\vone}{\mathbf{1}}
 \newcommand{\mystar}{{\fontfamily{lmr}\selectfont$\star$}}
\newcommand{\aucrelk}{\mbox{pAp}@k\xspace}
\newcommand{\pj}[1]{{\color{red} #1}}
\newcommand{\medres}{MEDRES\xspace}
\newcommand{\medreso}{MEDRES-P1\xspace}
\newcommand{\medrest}{MEDRES-P2\xspace}
\newcommand{\modifiedGCN}{AL-GCN\xspace}
\newcommand{\vGCN}{v-GCN\xspace}
\newcommand{\gcnp}{\modifiedGCN}
\newcommand{\medresM}{\modifiedGCN-MEDRES\xspace}
\newcommand{\medresV}{\vGCN-MEDRES\xspace}
%<<<<<<< HEAD
%\newcommand{\preck}{Precision@k\xspace}
%\newcommand{\pauc}{Partial-AUC\xspace}
%=======
\newcommand{\colf}{Collab\xspace}
\newcommand{\conf}{CoF\xspace}
%>>>>>>> 8145605cab92791f406e312603ea9e04ca5ba480


==> macros2.tex <==
% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{dsfont}
% \usepackage{amssymb,amsthm,commath}
% \usepackage{bm,xfrac,xcolor}
% \usepackage{nccmath}
% \usepackage[toc,page,header]{appendix}


% \usepackage{algorithm}
% \usepackage[noend]{algorithmic}
% \usepackage{bbm}
% \usepackage{enumitem}
% \usepackage{gensymb}
% \usepackage{refcount}
% \usepackage{mathtools}
% \usepackage{stackengine}

% \usetikzlibrary{calc}
% \usepackage{chngcntr}
% \counterwithout{equation}{section}
% \counterwithout{table}{section}
% \counterwithout{figure}{section}
% \counterwithout{algorithm}{section}
\usepackage{placeins,afterpage}

%---------------------------------------
% \usepackage[top=1in,bottom=1in,left=1in,right=1in]{geometry}
% \makeatletter
% \def\myfnt{\ifx\protect\@typeset@protect\expandafter\footnote\else\expandafter\@gobble\fi}
% \makeatother

% \makeatletter
% \def\BState{\State\hskip-\ALG@thistlm}
% \makeatother

% \makeatletter
% \newcommand*{\skipnumber}[2][1]{%
%   {\renewcommand*{\alglinenumber}[1]{}\State #2}%
%   \addtocounter{ALG@line}{-#1}}
% \makeatother

% \renewcommand\thealgorithm{}
% \makeatletter
% \newcommand{\setalglineno}[1]{%
%   \setcounter{ALC@line}{\numexpr#1-1}}
% \makeatother


% \renewcommand{\appendixpagename}{\centering Appendices}
% \newcommand\barbelow[1]{\stackunder[1.2pt]{$#1$}{\rule{1.5ex}{.1ex}}}
% \newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

% \DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand{\algorithmiccomment}[1]{\hfill\{\textit{#1}\}}


\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\Fig}[1]{Figure~\ref{#1}}
\newcommand{\Sec}[1]{Section~\ref{#1}}
\newcommand{\Tab}[1]{Table~\ref{#1}}
\newcommand{\Tabs}[2]{Tables~\ref{#1}--\ref{#2}}
\newcommand{\Eqn}[1]{Eq.~(\ref{#1})}
\newcommand{\Eqs}[2]{Eqs.~(\ref{#1}-\ref{#2})}
\newcommand{\Lem}[1]{Lemma~\ref{#1}}
\newcommand{\Thm}[1]{Theorem~\ref{#1}}
\newcommand{\Prop}[1]{Proposition~\ref{#1}}
\newcommand{\Cor}[1]{Corollary~\ref{#1}}
\newcommand{\App}[1]{Appendix~\ref{#1}}
\newcommand{\Def}[1]{Definition~\ref{#1}}

\newcommand{\tpr}{\textup{\textrm{TPR}}\xspace}
\newcommand{\fpr}{\textup{\textrm{FPR}}\xspace}
\newcommand{\tnr}{\textup{\textrm{TNR}}\xspace}
\newcommand{\fnr}{\textup{\textrm{FNR}}\xspace}

\newcommand{\reg}{\textup{\textrm{regret}}\xspace}
\newcommand{\er}{\textup{\textrm{er}}\xspace}
\newcommand{\auc}{\textup{\textrm{AUC}}\xspace}
\newcommand{\pauc}{\textup{\textrm{pAUC}}\xspace}
\newcommand{\partialauc}{\textup{\textrm{partial-AUC}}\xspace}

%\newcommand{\aucpreck}{\textup{\textrm{AUCprec@k}}}
\newcommand{\aucpreck}{\textup{\textrm{pAp@k}}\xspace}
\newcommand{\papk}{\textup{\textrm{pAp@k}}\xspace}

\newcommand{\preck}{\textup{\textrm{prec@k}}\xspace}
\newcommand{\precisionk}{\textup{\textrm{precision@k}}\xspace}
%\newcommand{\aucpk}{\textup{\textrm{AUCp@k}}\xspace}
\newcommand{\aucpk}{\textup{\textrm{pAp@k}}\xspace}

\newcommand{\svm}{\textup{\textrm{SVM}}\xspace}
\newcommand{\tight}{\textup{\textrm{tight}}\xspace}
\newcommand{\greedy}{\textup{\textrm{greedy}}\xspace}
\newcommand{\struct}{\textup{\textrm{struct}}\xspace}
%\newcommand{\tstruct}{\textup{\textrm{t-struct}}\xspace}
\newcommand{\tstruct}{\textup{\textrm{TS}}\xspace}
\newcommand{\ts}{\textup{\textrm{TS}}\xspace}
\newcommand{\dpauc}{\textup{\textrm{dpAUC}}\xspace}
\newcommand{\surr}{\textup{\textrm{surr}}\xspace}
\newcommand{\test}{\textup{\textrm{test}}\xspace}
\newcommand{\sign}{\textup{\textrm{sign}}\xspace}
\newcommand{\opt}{\textup{\textrm{opt}}\xspace}
\newcommand{\loss}{\textup{\textrm{loss}}\xspace}
\newcommand{\rank}{\textup{\textrm{rank}}\xspace}
\renewcommand{\dim}{\textup{\textrm{dim}}\xspace}
\newcommand{\zo}{\textup{\textrm{\scriptsize 0-1}}\xspace}
\newcommand{\extra}{\textup{\textrm{extra}}\xspace}
\newcommand{\hinge}{\textup{\textrm{hinge}}\xspace}
\newcommand{\ramp}{\textup{\textrm{ramp}}\xspace}
\newcommand{\maxi}{\textup{\textrm{max}}\xspace}
\newcommand{\avg}{\textup{\textrm{avg}}\xspace}

\newcommand{\maxisurr}{$\hat R^{\maxi}_\aucpreck(w;S)$}
\newcommand{\avgsurr}{$\hat R^{\avg}_\aucpreck(w;S)$}
\newcommand{\tstructsurr}{$\hat R^{\tstruct}_\aucpreck(w;S)$}
\newcommand{\structsurr}{$\hat R^{\struct}_\aucpreck(w;S)$}
\newcommand{\hingesurr}{$\hat R^{\hinge}_\aucpreck(w;S)$}

\newcommand{\gdmax}{GD-\papk-max\xspace}
\newcommand{\gdavg}{GD-\papk-avg\xspace}
\newcommand{\gdts}{GD-\papk-TS\xspace}
\newcommand{\svmpauc}{SVM-\pauc\xspace}
\newcommand{\sgdavg}{SGD@k-avg\xspace}
\newcommand{\greedypapk}{Greedy-\papk\xspace}

%\newcommand{\paucsurr}{$\hat R^{\tight}_\pauc(w;S)$}
%\newcommand{\precsurr}{$\hat R^{\avg}_\preck(w;S)$}
%\newcommand{\greedysurr}{$\hat R^{\greedy}_\papk(w;S)$}

\newcommand{\paucsurr}{\textup{\textrm{SVM-pAUC}}\xspace}
\newcommand{\precsurr}{\textup{\textrm{SGD@K-avg}}\xspace}
\newcommand{\greedysurr}{\textup{\textrm{greedy-pAp@k}}\xspace}

\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
% \renewcommand{\bar}{\widebar}
% \renewcommand{\breve}{\widebreve}

\newcommand{\rpm}{\sbox0{$1$}\sbox2{$\scriptstyle\pm$}
	\raise\dimexpr(\ht0-\ht2)/2\relax\box2 }


% \newcommand{\aucpreck}{AUCprec@k}
% \newcommand{\preck}{prec@k}

\newcommand{\TP}{\emph{TP}}
\newcommand{\TN}{\emph{TN}}
\newcommand{\FP}{\emph{FP}}
\newcommand{\FN}{\emph{FN}}

\newcommand{\TPs}{\emph{TP }}
\newcommand{\TNs}{\emph{TN }}
\newcommand{\FPs}{\emph{FP }}
\newcommand{\FNs}{\emph{FN }}

\newcommand{\Acal}{{\cal A}}
\newcommand{\Bcal}{{\cal B}}
\newcommand{\Ccal}{{\cal C}}
\newcommand{\Dcal}{{\cal D}}
\newcommand{\Ecal}{{\cal E}}
\newcommand{\Fcal}{{\cal F}}
\newcommand{\Gcal}{{\cal G}}
\newcommand{\Hcal}{{\cal H}}
\newcommand{\Ical}{{\cal I}}
\newcommand{\Jcal}{{\cal J}}
\newcommand{\Kcal}{{\cal K}}
\newcommand{\Lcal}{{\cal L}}
\newcommand{\Mcal}{{\cal M}}
\newcommand{\Ncal}{{\cal N}}
\newcommand{\Ocal}{{\cal O}}
\newcommand{\Pcal}{{\cal P}}
\newcommand{\Qcal}{{\cal Q}}
\newcommand{\Rcal}{{\cal R}}
\newcommand{\Scal}{{\cal S}}
\newcommand{\Tcal}{{\cal T}}
\newcommand{\Ucal}{{\cal U}}
\newcommand{\Vcal}{{\cal V}}
\newcommand{\Wcal}{{\cal W}}
\newcommand{\Xcal}{{\cal X}}
\newcommand{\Ycal}{{\cal Y}}
\newcommand{\Zcal}{{\cal Z}}


\newcommand{\Ambb}{\mathbb{A}}
\newcommand{\Bmbb}{\mathbb{B}}
\newcommand{\Cmbb}{\mathbb{C}}
\newcommand{\Dmbb}{\mathbb{D}}
\newcommand{\Embb}{\mathbb{E}}
\newcommand{\Fmbb}{\mathbb{F}}
\newcommand{\Gmbb}{\mathbb{G}}
\newcommand{\Hmbb}{\mathbb{H}}
\newcommand{\Imbb}{\mathbb{I}}
\newcommand{\Jmbb}{\mathbb{J}}
\newcommand{\Kmbb}{\mathbb{K}}
\newcommand{\Lmbb}{\mathbb{L}}
\newcommand{\Mmbb}{\mathbb{M}}
\newcommand{\Nmbb}{\mathbb{N}}
\newcommand{\Ombb}{\mathbb{O}}
\newcommand{\Pmbb}{\mathbb{P}}
\newcommand{\Qmbb}{\mathbb{Q}}
\newcommand{\Rmbb}{\mathbb{R}}
\newcommand{\Smbb}{\mathbb{S}}
\newcommand{\Tmbb}{\mathbb{T}}
\newcommand{\Umbb}{\mathbb{U}}
\newcommand{\Vmbb}{\mathbb{V}}
\newcommand{\Wmbb}{\mathbb{W}}
\newcommand{\Xmbb}{\mathbb{X}}
\newcommand{\Ymbb}{\mathbb{Y}}
\newcommand{\Zmbb}{\mathbb{Z}}


\newcommand{\Ambf}{\mathbf{A}}
\newcommand{\ambf}{\mathbf{a}}
\newcommand{\Bmbf}{\mathbf{B}}
\newcommand{\bmbf}{\mathbf{b}}
\newcommand{\Cmbf}{\mathbf{C}}
\newcommand{\cmbf}{\mathbf{c}}
\newcommand{\Dmbf}{\mathbf{D}}
\newcommand{\dmbf}{\mathbf{d}}
\newcommand{\Embf}{\mathbf{E}}
\newcommand{\embf}{\mathbf{e}}
\newcommand{\Fmbf}{\mathbf{F}}
\newcommand{\fmbf}{\mathbf{f}}
\newcommand{\Gmbf}{\mathbf{G}}
\newcommand{\gmbf}{\mathbf{g}}
\newcommand{\Hmbf}{\mathbf{H}}
\newcommand{\hmbf}{\mathbf{h}}
\newcommand{\Imbf}{\mathbf{I}}
\newcommand{\imbf}{\mathbf{i}}
\newcommand{\Jmbf}{\mathbf{J}}
\newcommand{\jmbf}{\mathbf{j}}
\newcommand{\Kmbf}{\mathbf{K}}
\newcommand{\kmbf}{\mathbf{k}}
\newcommand{\Lmbf}{\mathbf{L}}
\newcommand{\lmbf}{\mathbf{l}}
\newcommand{\Mmbf}{\mathbf{M}}
\newcommand{\mmbf}{\mathbf{m}}
\newcommand{\Nmbf}{\mathbf{N}}
\newcommand{\nmbf}{\mathbf{n}}
\newcommand{\Ombf}{\mathbf{O}}
\newcommand{\ombf}{\mathbf{o}}
\newcommand{\Pmbf}{\mathbf{P}}
\newcommand{\pmbf}{\mathbf{p}}
\newcommand{\Qmbf}{\mathbf{Q}}
\newcommand{\qmbf}{\mathbf{q}}
\newcommand{\Rmbf}{\mathbf{R}}
\newcommand{\rmbf}{\mathbf{r}}
\newcommand{\Smbf}{\mathbf{S}}
\newcommand{\smbf}{\mathbf{s}}
\newcommand{\Tmbf}{\mathbf{T}}
\newcommand{\tmbf}{\mathbf{t}}
\newcommand{\Umbf}{\mathbf{U}}
\newcommand{\umbf}{\mathbf{u}}
\newcommand{\Vmbf}{\mathbf{V}}
\newcommand{\vmbf}{\mathbf{v}}
\newcommand{\Wmbf}{\mathbf{W}}
\newcommand{\wmbf}{\mathbf{w}}
\newcommand{\Xmbf}{\mathbf{X}}
\newcommand{\xmbf}{\mathbf{x}}
\newcommand{\Ymbf}{\mathbf{Y}}
\newcommand{\ymbf}{\mathbf{y}}
\newcommand{\Zmbf}{\mathbf{Z}}
\newcommand{\zmbf}{\mathbf{z}}


\newcommand{\oline}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1}}
\newcommand{\Abar}{\oline{A}}
\newcommand{\abar}{\oline{a}}
\newcommand{\Bbar}{\oline{B}}
\newcommand{\bbar}{\oline{b}}
\newcommand{\Cbar}{\oline{C}}
\newcommand{\cbar}{\oline{c}}
\newcommand{\Dbar}{\oline{D}}
\newcommand{\dbar}{\oline{d}}
\newcommand{\Ebar}{\oline{E}}
\newcommand{\ebar}{\oline{e}}
\newcommand{\Fbar}{\oline{F}}
\newcommand{\fbar}{\oline{f}}
\newcommand{\Gbar}{\oline{G}}
\newcommand{\gbar}{\oline{g}}
\newcommand{\Hbar}{\oline{H}}
\renewcommand{\hbar}{\oline{h}}
\newcommand{\Ibar}{\oline{I}}
\newcommand{\ibar}{\oline{i}}
\newcommand{\Jbar}{\oline{J}}
\newcommand{\jbar}{\oline{j}}
\newcommand{\Kbar}{\oline{K}}
\newcommand{\kbar}{\oline{k}}
\newcommand{\Lbar}{\oline{L}}
\newcommand{\lbar}{\oline{l}}
\newcommand{\Mbar}{\skew{4}\overline{M}}
\newcommand{\mbar}{\oline{m}}
\newcommand{\Nbar}{\oline{N}}
\newcommand{\nbar}{\oline{n}}
\newcommand{\Obar}{\oline{O}}
\newcommand{\obar}{\oline{o}}
\newcommand{\Pbar}{\oline{P}}
\newcommand{\pbar}{\oline{p}}
\newcommand{\Qbar}{\oline{Q}}
\newcommand{\qbar}{\oline{q}}
\newcommand{\Rbar}{\oline{R}}
\newcommand{\rbar}{\oline{r}}
\newcommand{\Sbar}{\oline{S}}
\newcommand{\sbar}{\oline{s}}
\newcommand{\Tbar}{\oline{T}}
\newcommand{\tbar}{\oline{t}}
\newcommand{\Ubar}{\oline{U}}
\newcommand{\ubar}{\oline{u}}
\newcommand{\Vbar}{\oline{V}}
\newcommand{\vbar}{\oline{v}}
\newcommand{\Wbar}{\oline{W}}
\newcommand{\wbar}{\oline{w}}
\newcommand{\Xbar}{\oline{X}}
\newcommand{\xbar}{\oline{x}}
\newcommand{\Ybar}{\oline{Y}}
\newcommand{\ybar}{\oline{y}}
\newcommand{\zbar}{\oline{z}}
\newcommand{\Atilde}{\tilde{A}}
\newcommand{\atilde}{\tilde{a}}
\newcommand{\Btilde}{\tilde{B}}
\newcommand{\btilde}{\tilde{b}}
\newcommand{\Ctilde}{\tilde{C}}
\newcommand{\ctilde}{\tilde{c}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\dtilde}{\tilde{d}}
\newcommand{\Etilde}{\tilde{E}}
\newcommand{\etilde}{\tilde{e}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\ftilde}{\tilde{f}}
\newcommand{\Gtilde}{\tilde{G}}
\newcommand{\gtilde}{\tilde{g}}
\newcommand{\Htilde}{\tilde{H}}
\newcommand{\htilde}{\tilde{h}}
\newcommand{\Itilde}{\tilde{I}}
\newcommand{\itilde}{\tilde{i}}
\newcommand{\Jtilde}{\tilde{J}}
\newcommand{\jtilde}{\tilde{j}}
\newcommand{\Ktilde}{\tilde{K}}
\newcommand{\ktilde}{\tilde{k}}
\newcommand{\Ltilde}{\tilde{L}}
\newcommand{\ltilde}{\tilde{l}}
\newcommand{\Mtilde}{\tilde{M}}
\newcommand{\mtilde}{\tilde{m}}
\newcommand{\Ntilde}{\tilde{N}}
\newcommand{\ntilde}{\tilde{n}}
\newcommand{\Otilde}{\tilde{O}}
\newcommand{\otilde}{\tilde{o}}
\newcommand{\Ptilde}{\tilde{P}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\Qtilde}{\tilde{Q}}
\newcommand{\qtilde}{\tilde{q}}
\newcommand{\Rtilde}{\tilde{R}}
\newcommand{\rtilde}{\tilde{r}}
\newcommand{\Stilde}{\tilde{S}}
\newcommand{\stilde}{\tilde{s}}
\newcommand{\Ttilde}{\tilde{T}}
\newcommand{\ttilde}{\tilde{t}}
\newcommand{\Utilde}{\tilde{U}}
\newcommand{\utilde}{\tilde{u}}
\newcommand{\Vtilde}{\tilde{V}}
\newcommand{\vtilde}{\tilde{v}}
\newcommand{\Wtilde}{\tilde{W}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ztilde}{\tilde{Z}}
\newcommand{\ztilde}{\tilde{z}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\ahat}{\hat{a}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\chat}{\hat{c}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\khat}{\hat{k}}
\newcommand{\Lhat}{\widehat{L}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\phat}{\hat{p}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\shat}{\hat{s}}
\newcommand{\That}{\hat{T}}
\newcommand{\that}{\hat{t}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\What}{\hat{W}}
\newcommand{\what}{\hat{w}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\Zhat}{\hat{Z}}
\newcommand{\zhat}{\hat{z}}

\newcommand\inner[2]{\langle #1, #2 \rangle}
\newcommand{\Cdcal}{\mathcal{C}^{d}}
\newcommand{\Cd}{{C}^{d}}
\newcommand{\Cdistr}{C^d_{i\cancel{i}}}
\newcommand{\Cdonlyistr}{C^d_{\cancel{i}}}
\newcommand{\Cii}{C_{ii}}
\newcommand{\Cij}{C_{ij}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\hphi}{\hat{\phi}}

\newcommand{\bphi}{\oline{\phi}}
\newcommand{\bmmbf}{\oline{\mathbf{m}}}
\newcommand{\bmone}{\oline{m}_{11}}
\newcommand{\bmzero}{\oline{m}_{00}}
\newcommand{\bpone}{\oline{p}_{11}}
\newcommand{\bpzero}{\oline{p}_{00}}
\newcommand{\bqone}{\oline{q}_{11}}
\newcommand{\bqzero}{\oline{q}_{00}}
\newcommand{\bqnot}{\oline{q}_{0}}
\newcommand{\bell}{\oline{\ell}}
\newcommand{\btau}{\oline{\tau}}

%\newcommand{\hphi}{\hat{\phi}}
\newcommand{\hmmbf}{\hat{\mathbf{m}}}
\newcommand{\hmone}{\hat{m}_{11}}
\newcommand{\hmzero}{\hat{m}_{00}}
\newcommand{\hpone}{\hat{p}_{11}}
\newcommand{\hpzero}{\hat{p}_{00}}
\newcommand{\hqone}{\hat{q}_{11}}
\newcommand{\hqzero}{\hat{q}_{00}}
\newcommand{\hqnot}{\hat{q}_{0}}
\newcommand{\hell}{\hat{\ell}}

\newcommand{\sphi}{\phi^*}
\newcommand{\smmbf}{\mathbf{m}^*}
\newcommand{\smone}{{m_{11}^*}}
\newcommand{\smzero}{{m_{00}^*}}
\newcommand{\spone}{{p_{11}^*}}
\newcommand{\spzero}{{p_{00}^*}}
\newcommand{\sqone}{{q_{11}^*}}
\newcommand{\sqzero}{{q_{00}^*}}
\newcommand{\sqnot}{{q_{0}^*}}
\newcommand{\sell}{{\ell^*}}
\newcommand{\stau}{{\tau^*}}


\newcommand{\tphi}{\barbelow{\phi}}
\newcommand{\tmmbf}{\barbelow{\mathbf{m}}}
\newcommand{\tmone}{\barbelow{m}_{11}}
\newcommand{\tmzero}{\barbelow{m}_{00}}
\newcommand{\tpone}{\barbelow{p}_{11}}
\newcommand{\tpzero}{\barbelow{p}_{00}}
\newcommand{\tqone}{\barbelow{q}_{11}}
\newcommand{\tqzero}{\barbelow{q}_{00}}
\newcommand{\tqnot}{\barbelow{q}_{0}}
\newcommand{\tell}{\barbelow{\ell}}
\newcommand{\ttau}{\barbelow{\tau}}
\newcommand{\tC}{\barbelow{C}}

\newcommand{\pphi}{{\phi'}}
\newcommand{\pmmbf}{{\mathbf{m}'}}
\newcommand{\pmone}{{m}_{11}'}
\newcommand{\pmzero}{{m}_{00}'}
\newcommand{\ppone}{{p}_{11}'}
\newcommand{\ppzero}{{p}_{00}'}
\newcommand{\pqone}{{q}_{11}'}
\newcommand{\pqzero}{{q}_{00}'}
\newcommand{\pqnot}{{q}_{0}'}
\newcommand{\pell}{{\ell}'}
\newcommand{\ptau}{{\tau}'}

\newcommand{\ppphi}{{\phi''}}
\newcommand{\ppmmbf}{{\mathbf{m}''}}
\newcommand{\ppmone}{{m}_{11}''}
\newcommand{\ppmzero}{{m}_{00}''}
\newcommand{\pppone}{{p}_{11}''}
\newcommand{\pppzero}{{p}_{00}''}
\newcommand{\ppqone}{{q}_{11}''}
\newcommand{\ppqzero}{{q}_{00}''}
\newcommand{\ppqnot}{{q}_{0}''}
\newcommand{\ppell}{{\ell}''}
\newcommand{\pptau}{{\tau}''}

\DeclareMathOperator{\aff}      {aff}
\DeclareMathOperator{\cl}       {cl}
\DeclareMathOperator{\cone}     {cone}
\DeclareMathOperator{\coni}     {coni}
\DeclareMathOperator{\conv}     {conv}
\DeclareMathOperator{\dom}      {dom}
\DeclareMathOperator{\epi}      {epi}
\DeclareMathOperator{\inertia}  {inertia}
\DeclareMathOperator{\interior} {int}
\DeclareMathOperator{\linspan}  {span}
\DeclareMathOperator{\lin}      {lin}
\DeclareMathOperator{\minimize} {minimize}
\DeclareMathOperator{\Null}     {Null}
\DeclareMathOperator{\paraff}   {par}
\DeclareMathOperator{\proj}     {Proj}
\DeclareMathOperator{\recc}     {recc}
\DeclareMathOperator{\recf}     {recf}
\DeclareMathOperator{\ri}       {ri}
%\DeclareMathOperator{\st}       {s.\!t.}
\DeclareMathOperator{\subjectto}{subject~to}
\DeclareMathOperator{\trace}    {trace}
\DeclareMathOperator*{\argmin}   {arg\,min}
\DeclareMathOperator*{\argmax}   {arg\,max}
\DeclareMathOperator*{\arginf}   {arg\,inf}
\DeclareMathOperator*{\argsup}   {arg\,sup}


\newcommand{\half} {\frac12}
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\thalf}{\tfrac12}
\newcommand{\var}{{\mathbb{V}}}
\newcommand{\sgn}{\mbox{{sgn}}}
% Redefined math commands:
\renewcommand{\(}{\left)}
\renewcommand{\)}{\right)}
% Math commands with arguments
%\newcommand{\C}[1]{\mathbb{C}^{#1}}
\renewcommand{\E}{\mathbb{E}}
\newcommand{\eR}[1]{\skew{-2}\overline{\mathbb{R}}^{#1}}
\newcommand{\N}[1]{\mathbb{N}^{#1}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}[1]{\mathbb{Q}^{#1}}
\newcommand{\R}[1]{\mathbb{R}^{#1}}
\newcommand{\Z}[1]{\mathbb{Z}^{#1}}

\newcommand{\baligned}     {\begin{aligned}}
	\newcommand{\ealigned}     {\end{aligned}}
\newcommand{\barray}       {\begin{array}}
	\newcommand{\earray}       {\end{array}}
\newcommand{\bbmatrix}     {\begin{bmatrix}}
	\newcommand{\ebmatrix}     {\end{bmatrix}}
\newcommand{\bcases}       {\begin{cases}}
	\newcommand{\ecases}       {\end{cases}}
\newcommand{\bcenter}      {\begin{center}}
	\newcommand{\ecenter}      {\end{center}}
\newcommand{\bcolumn}      {\begin{column}}
	\newcommand{\ecolumn}      {\end{column}}
\newcommand{\bcolumns}     {\begin{columns}}
	\newcommand{\ecolumns}     {\end{columns}}
\newcommand{\benumerate}   {\begin{enumerate}}
	\newcommand{\eenumerate}   {\end{enumerate}}
\newcommand{\bequation}    {\begin{equation}}
	\newcommand{\eequation}    {\end{equation}}
\newcommand{\bequationn}   {\begin{equation*}}
	\newcommand{\eequationn}   {\end{equation*}}
\newcommand{\bfigure}      {\begin{figure}}
	\newcommand{\efigure}      {\end{figure}}
\newcommand{\bflushright}  {\begin{flushright}}
	\newcommand{\eflushright}  {\end{flushright}}
\newcommand{\bitemize}     {\begin{itemize}}
	\newcommand{\eitemize}     {\end{itemize}}
\newcommand{\bpmatrix}     {\begin{pmatrix}}
	\newcommand{\epmatrix}     {\end{pmatrix}}
\newcommand{\bsubequations}{\begin{subequations}}
	\newcommand{\esubequations}{\end{subequations}}
\newcommand{\btable}       {\begin{table}}
	\newcommand{\etable}       {\end{table}}
\newcommand{\btabular}     {\begin{tabular}}
	\newcommand{\etabular}     {\end{tabular}}
\newcommand{\bvmatrix}     {\begin{vmatrix}}
	\newcommand{\evmatrix}     {\end{vmatrix}}

\newcommand{\bequalin}     {\bequationn\baligned}
\newcommand{\eequalin}     {\ealigned\eequationn}
\newcommand{\bequali}      {\bsubequations\begin{align}}
	\newcommand{\eequali}      {\end{align}\esubequations}


\newtheorem{assumption}{Assumption}
\newtheorem{prop}{Proposition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}

\newcommand{\balgorithm}  {\begin{algorithm}}
	\newcommand{\ealgorithm}  {\end{algorithm}}
\newcommand{\balgorithmic}{\begin{algorithmic}}
	\newcommand{\ealgorithmic}{\end{algorithmic}}
\newcommand{\bassumption} {\begin{assumption}}
	\newcommand{\eassumption} {\end{assumption}}
\newcommand{\bcorollary}  {\begin{corollary}}
	\newcommand{\ecorollary}  {\end{corollary}}
\newcommand{\bdefinition} {\begin{definition}}
	\newcommand{\edefinition} {\end{definition}}
\newcommand{\bexample}    {\begin{example}}
	\newcommand{\eexample}    {\end{example}}
\newcommand{\bproposition}    {\begin{prop}}
	\newcommand{\eproposition}    {\end{prop}}
\newcommand{\blemma}      {\begin{lemma}}
	\newcommand{\elemma}      {\end{lemma}}
\newcommand{\bproblem}    {\begin{problem}}
	\newcommand{\eproblem}    {\end{problem}}
\newcommand{\bproof}      {\begin{proof}}
	\newcommand{\eproof}      {\end{proof}}
\newcommand{\bremark}     {\begin{remark}}
	\newcommand{\eremark}     {\end{remark}}
\newcommand{\btheorem}    {\begin{theorem}}
	\newcommand{\etheorem}    {\end{theorem}}

\renewcommand\theadalign{bl}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\theadfont{\tiny}
\renewcommand\cellgape{\Gape[4pt]}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\bc}[1]{\left\{{#1}\right\}}
\newcommand{\br}[1]{\left({#1}\right)}
\newcommand{\bs}[1]{\left[{#1}\right]}
% \newcommand{\abs}[1]{\left| {#1} \right|}
% \newcommand{\norm}[1]{\left\| {#1} \right\|}
% \newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
% \newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\bsd}[1]{\left\llbracket{#1}\right\rrbracket}

% \algrenewcommand\algorithmicindent{0.1cm}%

